Neural Garment Dynamic Super-Resolution

Achieving efficient, high-fidelity, high-resolution garment simulation is challenging due to its computational demands. Conversely, low-resolution garment simulation is more accessible and ideal for low-budget devices like smartphones. In this paper, we introduce a lightweight, learning-based method for garment dynamic super-resolution, designed to efficiently enhance high-resolution, high-frequency details in low-resolution garment simulations. Starting with low-resolution garment simulation and underlying body motion, we utilize a mesh-graph-net to compute super-resolution features based on coarse garment dynamics and garment-body interactions. These features are then used by a hyper-net to construct an implicit function of detailed wrinkle residuals for each coarse mesh triangle. Considering the influence of coarse garment shapes on detailed wrinkle performance, we correct the coarse garment shape and predict detailed wrinkle residuals using these implicit functions. Finally, we generate detailed high-resolution garment geometry by applying the detailed wrinkle residuals to the corrected coarse garment. Our method enables roll-out prediction by iteratively using its predictions as input for subsequent frames, producing fine-grained wrinkle details to enhance the low-resolution simulation. Despite training on a small dataset, our network robustly generalizes to different body shapes, motions, and garment types not present in the training data. We demonstrate significant improvements over state-of-the-art alternatives, particularly in enhancing the quality of high-frequency, fine-grained wrinkle details.

==> 8_figs.tex <==
\begin{figure*}[!htbp]
    \centering
    % \includegraphics[width=0.87\textwidth]{fig/asia/rst_seen_garments_ad.pdf}
    \includegraphics[width=0.87\textwidth]{fig/asia_final/rst_seen_garments_ad.pdf}
    \vskip -0.15in
    \caption{ We run our method by roll-out prediction on both seen (1st row) and unseen (2nd row) motions with the training garment types. For each example, we show input of low resolution simulation, results of coarse shape correction and detailed high resolution results,  as well as the reference of high resolution simulation.}
    % \caption{\textbf{Seen garment results.} 
    % Training with the long skirt on a fixed body shape, our GDSR-A can generalize across out-of-training motions, different garment types (tunics and lace skirt, t-shirt and long pants), and unseen body shapes (dressing on t-shirt and long pants). GDSR-A produces 3D high-resolution garment geometry with rich yet plausible wrinkle details.}
    \label{fig:seen_garments}
\end{figure*}


\begin{figure*}[!htbp]
    \centering
    % \includegraphics[width=0.90\textwidth]{fig/asia/rst_unseen_garments_ad.pdf}
    \includegraphics[width=0.90\textwidth]{fig/asia_final/rst_unseen_garments_ad.pdf}
    \vskip -0.15in
    \caption{We evaluate the generalization of our method on motions and garment types that are both out of the training data. Our method can synthesize fine-grained wrinkle details for either single- or multi-layer garments.}
    % \caption{\textbf{Unseen garment results.} 
    % Given the low resolution garment dynamics and the underlying body motion, our GDSR-B jointly corrects the coarse garment shape and produces fine wrinkle details to synthesis high fidelity, high resolution garment meshes. Although the network is trained garment specific with a fixed body shape, GDSR-B can generalize across out-of-training body motions and body shapes. We enable the generalization across unseen garments by fine-tuning the network. Here, we show the performance of GDSR-B on a multi-layer dress and a pleated skirt.}
    \label{fig:unseen_garments}
\end{figure*}

% \begin{figure}[h!]
%    \includegraphics[width=\columnwidth]{fig/tSNT-5motion.pdf}
%  \vskip -0.1in
%    \centering
%    \caption{
%     We visualize the distribution of dancing sequences used as training data (\emph{House} and \emph{Swing}) and testing data (\emph{Salsa}, \emph{Samba}, and \emph{Samba variation}) via t-SNE \cite{van2008visualizing}. 
%     %There is little overlapping between the distributions of the training and testing motions.
%   }
%    \label{fig:tSNE}
%     %\vskip -0.1in
%  \end{figure}

\begin{figure*}[!htbp]
   \centering
   % \includegraphics[width=0.90\textwidth]{fig/asia/rst_unseen_bodyshapes_ad.pdf}
   \includegraphics[width=0.90\textwidth]{fig/asia_final/rst_unseen_bodyshapes_ad.pdf}
       \vskip -0.15in
   \caption{
    We evaluate the generalization of our method across different body shapes on out-of-training motions with both seen and unseen garment types. 
    Although trained with a fixed body shape, our method can synthesize detailed high-resolution garment geometry fitting with varying body shapes. 
  }
   \label{fig:bodyshape}
 \end{figure*}


 \begin{figure}[!htpb]
   \centering
   % \includegraphics[width=\columnwidth]{fig/asia/long_walking_ad.pdf}
   \includegraphics[width=\columnwidth]{fig/asia_final/long_walking_ad.pdf}
       \vskip -0.1in
   \caption{
    We evaluate the robustness of our method under long roll-out predictions up to 1500 frames, using a seen garment (in purple and yellow) and an unseen garment (in teal and pink) with happy walking and normal walking motion sequences, respectively. Our method uses low-resolution simulation and its predictions as input for subsequent frames to produce reasonable wrinkle details while maintaining plausible temporal smoothness between frames.
  }
   \label{fig:longrollout}
 \end{figure}

 
\begin{figure}[!htpb]
   \centering
    % \includegraphics[width=0.95\columnwidth]{fig/asia/coarse_effect_1.pdf}
    \includegraphics[width=0.95\columnwidth]{fig/asia_final/coarse_effect_1.pdf}
    \vskip -0.1in
    \caption{
    To evaluate the effect of coarse garment correction, we designed two variants of GDSR by removing the \emph{Decoder} $\mathcal{E}$, named GDSR(-r) and GDSR(-d) respectively. Our full model of GDSR produces remarkably fine-grained high-resolution garment geometry with wrinkle detail patterns similar to the reference of high-resolution simulation, compared to GDSR(-r), which does not consider the influence of coarse garment shape, and GDSR(-d), which relies on roll-out prediction but without correcting the garment shape at coarse level.}
    
    %To evaluate the effect of coarse garment correction, we design two variants of GDSR by removing the \emph{Decoder} $\mathcal{E}$, named as GDSR(-r) and GDSR(-d) respectively. Our full model of GDSR produces remarkable fine-grained HR garment geometry with wrinkle detail patterns similar to the reference HR simulation, comparing with the result of GDSR(-r) without considering the influence of coarse garment shape, as well as the result of GDSR(-d) produced by roll-out prediction with only \emph{Mesh-Graph-Net} $\mathcal{H}$ and \emph{Decoder} $\mathcal{A}$.
    
    \label{fig:coarse_correction}
\end{figure}


\begin{figure}[!htpb]
   \centering
    % \includegraphics[width=1\columnwidth]{fig/asia/comparison_ad.pdf}
    % \includegraphics[width=1\columnwidth]{fig/asia/comparisons_more.png}
    \includegraphics[width=1\columnwidth]{fig/asia_final/comparison_ad_threerow.pdf}
    \vskip -0.1in
    \caption{Given the low-resolution simulation garment geometry, our GDSR constructs the high-resolution garment geometry by synthesizing fine detail wrinkles, applied on the corrected coarse garment mesh. Comparing to PhysGraph \cite{halimi2023physgraph} and DDE\cite{zhang2021deep}, GDSR captures fine-grained wrinkle patterns more similar to the reference high-resolution simulation.}
    \label{fig:comparisons}
\end{figure}


\begin{figure}[!htpb]
   \centering
    % \includegraphics[width=\columnwidth]{fig/asia/limitation_ad.pdf}
    \includegraphics[width=\columnwidth]{fig/asia_final/limitation_ad.pdf}
    \vskip -0.1in
    \caption{\textbf{Limitation.} Our method fails to capture garment details influenced by friction between fabric layers. Although our explicit collision handling resolves most intersections between fabric layers, some collisions remain because we cannot detect intersections when the distances between intersecting vertices exceed the predefined threshold.}
    \label{fig:limitation}
\end{figure}


% \begin{figure}
%    \includegraphics[width=\columnwidth]{fig/roll-out.pdf}
%     \vskip -0.2in
%    \centering
%    \caption{
%    We test the stability of GDSR-B rollout prediction. We visualize the L2 error between the prediction and the high-resolution simulation ground truth, varying with the frame index. The error increases with iteration at the beginning, then oscillates within a controllable range. 
%     % We visualize the distribution of dancing sequences used as training data (\emph{House} and \emph{Swing}) and testing data (\emph{Salsa}, \emph{Samba}, and \emph{Samba variation}) via t-SNE \cite{van2008visualizing}. 
%     %There is little overlapping between the distributions of the training and testing motions.
%   }
%    \label{fig:rollout}
%     \vskip -0.1in
%  \end{figure}

% \begin{figure}
%    \includegraphics[width=0.7\columnwidth]{fig/tSNT-5motion.pdf}
%        % \vskip -0.1in
%    \centering
%    \caption{
%     We visualize the distribution of dancing sequences used as training data (\emph{House} and \emph{Swing}) and testing data (\emph{Salsa}, \emph{Samba}, and \emph{Samba variation}) via t-SNE \cite{van2008visualizing}. 
%     %There is little overlapping between the distributions of the training and testing motions.
%   }
%    \label{fig:tSNE}
%  \end{figure}
